Multiplicative Properties of the Slice Filtration

We show that the slice filtration introduced by Voevodsky is compatible in a suitable sense with the symmetric monoidal structure in the category of motivic symmetric T-spectra constructed by Jardine. It follows from this compatibility that the zero slice of the sphere spectrum s_{0}(1) is a ring spectrum and that for every symmetric T-spectrum X, and every integer n; the n-slice s_{n}(X) is a module over s_{0}(1). In particular, if the base scheme is a field of characteristic zero, we have that all the slices s_{n}(X) are big motives in the sense of Voevodsky. We also get as a corollary that the smash product of symmetric T-spectra induces pairings in the motivic Atiyah-Hirzebruch spectral sequence.

==> chapters/abstract.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{abstract}
	
	Let $S$ be a Noetherian separated scheme of finite dimension.
	In \cite{MR1977582}, Voevodsky constructs the slice filtration in the motivic
	stable homotopy category $\stablehomotopy$, as an analogue to the Postnikov
	tower in algebraic topology.  Our main results show that for every
	symmetric $T$-spectrum $X$, the direct sum of all the slices
	$s^{\Sigma}(X)=\oplus _{n\in \mathbb Z}s_{n}^{\Sigma}X$
	has the structure of a graded module over
	$s^{\Sigma}(\symmspherespectrum )=\oplus _{n\in \mathbb Z}s_{n}^{\Sigma}\symmspherespectrum$, 
	where $\symmspherespectrum$ denotes the
	sphere spectrum.  Furthermore, if the base scheme
	$S$ is a perfect field then we show that all the slices $s_{n}^{\Sigma}X$ are big
	motives in the sense of Voevodsky.
\end{abstract}

==> chapters/sections-1/subsect-1.1/subsect-derivfunct.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{section}{Derived Functors}
		\label{subsec-derivedfunctors}
		
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
\begin{defi}
		\label{def.1.2.adjointfunct}
	Let $\mathcal{C,D}$ be two categories.
	An \emph{adjunction} from $\mathcal C$ to $\mathcal D$
	consists of a triple $(F,G,\varphi)$,
	where $F:\mathcal C \rightarrow \mathcal D$,
	$G:\mathcal D \rightarrow \mathcal C$ are functors
	and $\varphi$ is a natural isomorphism between
	the following bifunctors:
	$$\xymatrix@R=.5pt{\mathcal C ^{op}\times \mathcal D \ar[rr]^-{F\times id}&& 
							\mathcal D ^{op}\times \mathcal D \ar[rr]^-{\Hom _{\mathcal D}(-,-)}&& Sets\\
							\mathcal C ^{op}\times \mathcal D \ar[rr]_-{id\times G}&& 
							\mathcal C ^{op}\times \mathcal C \ar[rr]_-{\Hom_{\mathcal C}(-,-)}&& Sets}
	$$
	i.e. for any pair of objects $X\in \mathcal C$
	and $Y\in \mathcal D$ we have a natural bijection
	$\varphi_{X,Y}:\Hom _{\mathcal D}(FX,Y)\rightarrow \Hom _{\mathcal C}(X,GY)$.
	The functor $F$ is called a \emph{left adjoint} and the functor
	$G$ is called a \emph{right adjoint}.
\end{defi}

%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%
\begin{defi}[cf. \cite{MR0223432}*{I.4 definition 1}]
		\label{def.1.2.leftderived-functors}
	Consider the following diagram where
	$\gamma$ and $F$ are functors:
	$$\xymatrix{\mathcal A \ar[r]^-{F} \ar[d]_{\gamma}& \mathcal C \\
							\mathcal B}
	$$
	The \emph{left derived functor} of $F$ with respect to $\gamma$
	is a functor $\mathbf{L}F:\mathcal B \rightarrow \mathcal C$ together
	with a natural transformation $\epsilon :\mathbf{L}F\circ \gamma \rightarrow F$
	having the following universal property:
	given any functor $G:\mathcal B \rightarrow \mathcal C$ together with a
	natural transformation $\delta :G\circ \gamma \rightarrow F$ there is a unique
	natural transformation $\theta :G\rightarrow \mathbf{L}F$ such that the 
	following diagram of natural transformations commutes:
	$$\xymatrix{G\circ \gamma \ar[r]^-{\delta} \ar[d]_-{\theta _{\gamma}}& F\\
							\mathbf{L}F\circ \gamma \ar[ur]_-{\epsilon}& }
	$$	
\end{defi}

%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%
\begin{defi}
		\label{def.1.2.rightderived-functors}
	Consider the following diagram where
	$\gamma$ and $F$ are functors:
	$$\xymatrix{\mathcal A \ar[r]^-{F} \ar[d]_{\gamma}& \mathcal C \\
							\mathcal B}
	$$
	The \emph{right derived functor} of $F$ with respect to $\gamma$
	is a functor $\mathbf{R}F:\mathcal B \rightarrow \mathcal C$ together
	with a natural transformation $\epsilon :F\rightarrow \mathbf{R}F\circ \gamma$
	having the following universal property:
	given any functor $G:\mathcal B \rightarrow \mathcal C$ together with a
	natural transformation $\delta :F\rightarrow G\circ \gamma$ there is a unique
	natural transformation $\theta :\mathbf{R}F\rightarrow G$ such that the 
	following diagram of natural transformations commutes:
	$$\xymatrix{F \ar[r]^-{\epsilon} \ar[dr]_-{\delta}& \mathbf{R}F\circ \gamma  \ar[d]^-{\theta _{\gamma}} \\
							& G\circ \gamma  }
	$$	
\end{defi}

%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%
\begin{defi}
		\label{def.1.2.der-func-wrt-modcats}
	Let $F:\modelcat \rightarrow \mathcal D$ be a functor,
	where $\modelcat$ is a model category.
	\begin{enumerate}
		\item	A \emph{left derived functor} of $F$ is a functor
					$$\mathbf{L}F:\hocat \rightarrow \mathcal D$$ together
					with a natural transformation $\epsilon :\mathbf{L}F\circ \gamma \rightarrow F$
					such that the pair $(\mathbf{L}F,\epsilon)$ is ``closest to $F$ from the left'',
					i.e. such that if $G:\hocat \rightarrow \mathcal D$ is a functor and
					$\delta :G\circ \gamma \rightarrow F$ is a natural transformation, then
					there is a unique natural transformation $\theta :G\rightarrow \mathbf{L}F$
					such that $\delta =\epsilon(\theta \circ \gamma)$.
		\item	A \emph{right derived functor} of $F$ is a functor
					$$\mathbf{R}F:\hocat \rightarrow \mathcal D$$ together
					with a natural transformation $\epsilon :F\rightarrow \mathbf{R}F\circ \gamma$
					such that the pair $(\mathbf{R}F,\epsilon)$ is ``closest to $F$ from the right'',
					i.e. such that if $G:\hocat \rightarrow \mathcal D$ is a functor and
					$\delta:F \rightarrow G\circ \gamma$ is a natural transformation, then
					there is a unique natural transformation $\theta :\mathbf{R}F\rightarrow G$ such
					that $\delta =(\theta \circ \gamma)\epsilon$.
	\end{enumerate}
\end{defi}

	The left derived functor of $F$ is also known as the right Kan extension
	of $F$ along $\gamma :\modelcat \rightarrow \hocat$.  Similarly,
	the right derived functor of $F$ is also known as the left Kan extension
	of $F$ along $\gamma :\modelcat \rightarrow \hocat$.

%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%
\begin{prop}
		\label{prop1.2.existence-derfunc}
	Let $F:\modelcat \rightarrow \mathcal D$ be a functor where
	$\modelcat$ is a model category.
	\begin{enumerate}
		\item	If $F$ maps trivial cofibrations between cofibrant objects
					to isomorphisms in $\mathcal D$, then the left derived
					functor $\mathbf{L}F$ of $F$ exists.
		\item	If $F$ maps trivial fibrations between fibrant objects
					to isomorphisms in $\mathcal D$, then the right derived
					functor $\mathbf{R}F$ of $F$ exists.
	\end{enumerate}
\end{prop}

%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%
\begin{defi}
		\label{def.1.2.totderfunct}
	Let $\modelcat$, $\modelcattwo$ be model categories a let
	$F:\modelcat \rightarrow \modelcattwo$ be a functor.
	\begin{enumerate}
		\item	The \emph{total left derived functor} of $F$ is the left
					derived functor of the composition
					$$\xymatrix{\modelcat \ar[r]^-{F}& \modelcattwo \ar[r]^-{\gamma_{\modelcattwo}}& \hocattwo}$$
					with respect to the localization $\gamma _{\modelcat}:\modelcat \rightarrow \hocat$.
		\item The \emph{total right derived functor} of $F$ is the right
					derived functor of the composition
					$$\xymatrix{\modelcat \ar[r]^-{F}& \modelcattwo \ar[r]^-{\gamma _{\modelcattwo}}& \hocattwo}$$
					with respect to the localization $\gamma _{\modelcat}:\modelcat \rightarrow \hocat$.
	\end{enumerate}
\end{defi}

%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%
\begin{cor}
		\label{cor.1.2.totderfunct-existence}
	Let $F:\modelcat \rightarrow \modelcattwo$ be a functor
	between two model categories.
	\begin{enumerate}
		\item	If $F$ takes trivial cofibrations between cofibrant objects
					in $\modelcat$ into weak equivalences in $\modelcattwo$,
					then the total left derived functor $\mathbf{L}F:\hocat \rightarrow \hocattwo$
					exists.
		\item	If $F$ takes trivial fibrations between fibrant objects
					in $\modelcat$ into weak equivalences in $\modelcattwo$,
					then the total right derived functor
					$\mathbf{R}F:\hocat \rightarrow \hocattwo$ exists.
	\end{enumerate}
\end{cor}

%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%
\begin{defi}
		\label{def.1.2.Quillenfunctors}
	Let $\modelcat$, $\mathcal N$ be two model categories.
	A functor $F:\modelcat \rightarrow \mathcal N$ is called
	a \emph{left Quillen functor} if it has a right adjoint
	$G:\mathcal N \rightarrow \modelcat$, and satisfies
	the following conditions:
	\begin{enumerate}
		\item	If $i$ is a cofibration in $\modelcat$,
					then $F(i)$ is also a cofibration in $\mathcal N$.
		\item	If $j$ is a trivial cofibration in $\modelcat$,
					then $F(j)$ is also a trivial cofibration
					in $\mathcal N$.
	\end{enumerate}
	The right adjoint $G$ is called a
	\emph{right Quillen functor},
	and the adjunction $(F,G,\varphi):\modelcat \rightarrow \modelcattwo$
	is called a \emph{Quillen adjunction}.
\end{defi}

	The following statement is an easy consequence of the definitions.
	
%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{rmk}
		\label{rmk.1.2.Quillenfunctors}
	Let $(F,G,\varphi):\modelcat \rightarrow \modelcattwo$ be an adjunction
	between two model categories.
	Then the following are equivalent:
	\begin{enumerate}
		\item	$F$ is a left Quillen functor.
		\item	$G$ satisfies the following two conditions:
					\begin{enumerate}
						\item	If $p$ is a fibration in $\modelcattwo$,
									then $G(p)$ is also a fibration in $\modelcat$.
						\item	If $q$ is a trivial fibration in $\modelcattwo$,
									then $G(q)$ is also a trivial fibration in $\modelcat$.
					\end{enumerate}
		\item	$F$ and $G$ satisfy the following conditions:
					\begin{enumerate}
						\item	If $i$ is a cofibration in $\modelcat$,
									then $F(i)$ is also a cofibration in $\modelcattwo$.
						\item	If $p$ is a fibration in $\modelcattwo$,
									then $G(p)$ is also a fibration in $\modelcat$.
					\end{enumerate}
		\item	$F$ and $G$ satisfy the following conditions:
					\begin{enumerate}
						\item	If $j$ is a trivial cofibration in $\modelcat$,
									then $F(j)$ is also a trivial cofibration in $\modelcattwo$.
						\item	If $q$ is a trivial fibration in $\modelcattwo$,
									then $G(q)$ is also a trivial fibration in $\modelcat$.
					\end{enumerate}
	\end{enumerate}
\end{rmk}

%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{prop}[Dugger, cf. \cite{MR1944041}]
		\label{prop1.2.criterion-leftQuillen-functors}
	Let $(F,G,\varphi):\modelcat \rightarrow \modelcattwo$ be an adjunction
	between two model categories.
	Then the following are equivalent:
	\begin{enumerate}
		\item	\label{prop1.2.criterion-leftQuillen-functors.a}$F$ is a left Quillen functor.
		\item	\label{prop1.2.criterion-leftQuillen-functors.b}$F$ preserves cofibrations between cofibrant objects and all 
					trivial cofibrations.
		\item	\label{prop1.2.criterion-leftQuillen-functors.c}$G$ preserves fibrations between fibrant objects and all
					trivial fibrations.
	\end{enumerate}
\end{prop}
\begin{proof}
	It is obvious that condition (\ref{prop1.2.criterion-leftQuillen-functors.a}) implies
	(\ref{prop1.2.criterion-leftQuillen-functors.b}) and (\ref{prop1.2.criterion-leftQuillen-functors.c}).
	By duality it is enough to show that
	(\ref{prop1.2.criterion-leftQuillen-functors.b}) implies (\ref{prop1.2.criterion-leftQuillen-functors.a}).
	Suppose then that $F$ preserves cofibrations between cofibrant objects and  trivial cofibrations,
	remark \ref{rmk.1.2.Quillenfunctors} implies that it is enough to show that $G$ preserves
	trivial fibrations.  Since $F$,$G$ are adjoint and $F$ preserves
	trivial cofibrations, the characterizaction of fibrations via a lifting property
	implies that $G$ preserves fibrations.
	Let $q:X\rightarrow Y$ be a trivial fibration in $\modelcattwo$, so
	$q$ is in particular a fibration, and then it follows that $G(q)$
	is also a fibration in $\modelcat$.  It only remains to show
	that $G(q)$ is a weak equivalence.
	The factorization axiom $\mathbf{MC5}$ implies that it is
	posibble to find a cofibrant approximation for $G(q)$
	$$\xymatrix{A \ar[r]^-{p_{X}} \ar[d]_-{i}& GX \ar[d]^-{G(q)}\\
							B \ar[r]_-{p_{Y}}& GY}
	$$
	where $A,B$ are cofibrant, $p_{X},p_{Y}$ are trivial fibrations and
	$i$ is a cofibration.  The two out of three property for weak equivalences
	implies that it is enough to show that $i$ is a weak equivalence.
	The adjunction gives the following commutative diagram in $\modelcattwo$
	$$\xymatrix{FA \ar[r]^-{{p_{X}}^{\sharp}} \ar[d]_-{F(i)}& X \ar[d]^-{q}\\
							FB \ar[r]_-{{p_{Y}}^{\sharp}} \ar@{-->}[ur]^-{s}& Y}
	$$
	The dotted arrow making the diagram commutative exists, since $F$ preserves
	cofibrations between cofibrant objects and by hypothesis $q$ is a trivial fibration.
	Using the adjunction again we get the following commutative diagram
	$$\xymatrix{A \ar[r]^-{p_{X}} \ar[d]_-{i}& GX \ar[d]^-{G(q)}\\
							B \ar[r]_-{p_{Y}} \ar[ur]_-{s_{\sharp}}& GY}
	$$
	Now since $i$ is a cofibraton and $p_{X}$ is a trivial fibration,
	we have a lifting in the diagram
	$$\xymatrix{A \ar[r]^-{id} \ar[d]_-{i}& A \ar[d]^-{p_{X}}\\
							B \ar[r]_-{s_{\sharp}} \ar@{-->}[ur]^-{r}& GX}
	$$
	so $ri=id_{A}$, this implies that $[r][i]=id_{A}$ in $\hocat$.
	It is enough to show that $[i][r]=id_{B}$ in $\hocat$ since 
	maps which become isomorphisms in $\hocat$ are forced to be
	weak equivalences.  But
	$p_{Y}ir=G(q)p_{X}r=G(q)s_{\sharp}=p_{Y}=p_{Y}id_{B}$, and since
	$p_{Y}$ is a trivial fibration lemma \ref{lem1.1.trivfib=>iso-on=homgrps}
	implies that $ir\stackrel{l}{\sim}id_{B}$, hence
	$[i][r]=id_{B}$ in $\hocat$.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{prop}
		\label{prop.1.2.Quillen-adjunction=>descends}
	Let $(F,G,\varphi):\modelcat \rightarrow \modelcattwo$ be a Quillen
	adjunction.  Then the adjunction $(F,G,\varphi)$ descends to the homotopy categories, i.e.
	we get an adjuntion:
	$(\mathbf{L}F,\mathbf{R}F,\varphi):\hocat \rightarrow \hocattwo$.
\end{prop}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{defi}
		\label{def.1.2.Quillen-equiv}
	Let $(F,G,\varphi):\modelcat \rightarrow \modelcattwo$ be a Quillen adjunction.
	We say that $F$ is a \emph{left Quillen equivalence} if
	for every cofibrant object $A$ in $\modelcat$ and every
	fibrant object $X$ in $\modelcattwo$ the following condition holds:
	\begin{itemize}
		\item	A map $f:A\rightarrow GX$ is a weak equivalence in $\modelcat$
					if and  only if its adjoint $f^{\sharp}:FA\rightarrow X$
					is a weak equivalence in $\modelcattwo$.
	\end{itemize}
	In this case $G$ will be called a \emph{right Quillen equivalence}, and
	$(F,G,\varphi)$ a \emph{Quillen equivalence}.
\end{defi}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{prop}
		\label{prop1.2.Quillenequiv=>Homotequiv}
	Let $(F,G,\varphi):\modelcat \rightarrow \modelcattwo$ be a Quillen adjunction.
	The following are equivalent:
	\begin{enumerate}
		\item	$(F,G,\varphi)$ is a Quillen equivalence.
		\item	For any cofibrant object $A$ in $\modelcat$ the map
					$$\xymatrix{A \ar[rr]^-{\eta}&& GFA \ar[rr]^-{G(r_{FA})}&& GRFA}
					$$
					is a weak equivalence, and for any fibrant object $X$ in $\modelcattwo$
					the map
					$$\xymatrix{FQGX \ar[rr]^-{F(q_{GX})}&& FGX \ar[rr]^-{\epsilon} && X}
					$$
					is a weak equivalence.
		\item	$(\mathbf{L}F, \mathbf{R}G, \varphi)$ is an equivalence of categories.
	\end{enumerate} 
\end{prop}

	A functor $F$ is said to \emph{reflect} some property if
	given a map $f$ such that $F(f)$ has the property then
	$f$ has also the property.
	
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{prop}
		\label{prop1.2.classQuillenequiv}
	Let $(F,G,\varphi):\modelcat \rightarrow \modelcattwo$ be a Quillen
	adjunction.  The following are equivalent:
	\begin{enumerate}
		\item	$(F,G,\varphi)$ is a Quillen equivalence.
		\item	$F$ reflects weak equivalences between cofibrant objects, and for
					every fibrant object $X$ in $\modelcattwo$, the map
					$$\xymatrix{FQGX \ar[rr]^-{F(q_{GX})}&& FGX \ar[rr]^-{\epsilon} && X}
					$$
					is a weak equivalence.
		\item	$G$ reflects weak equivalences between fibrant objects, and for
					every cofibrant object $A$ in $\modelcat$, the map
					$$\xymatrix{A \ar[rr]^-{\eta}&& GFA \ar[rr]^-{G(r_{FA})}&& GRFA}
					$$
					is a weak equivalence.
	\end{enumerate}
\end{prop}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{prop}
		\label{prop1.2.derivedadjunc-iso-conditions}
	Let $\tau :F\rightarrow G$ be a natural transformation between
	left (respectively right) Quillen functors.  Then
	$\mathbf{L}\tau$ (respectively $\mathbf{R}\tau$) is a natural
	isomorphism if and only if $\tau_{X}$ is a weak equivalence
	for all cofibrant (respectively fibrant) $X$.
\end{prop}
\end{section}

==> chapters/sections-1/subsect-1.1/subsect-homotcat.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{section}{The homotopy category}
		\label{subsect-homotcat}
		
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{defi}
		\label{def.1.1.cylinderobject}
	Let $\modelcat$ be a model category, and let $A$ be an object of $\modelcat$.
	We say that $\tilde{A}$ is a \emph{cylinder object} for $A$, if we have a
	factorization of the fold map
	$$\xymatrix{A\coprod A \ar[r]^-{\nabla} \ar[d]_-{i} & A\\
							\tilde{A} \ar[ur]_-{s}&}
	$$
	where $i$ is a cofibration and $s$ is a weak equivalence.
\end{defi}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{defi}
		\label{def.1.1.lefthomotopy}
	Let $\modelcat$ be a model category and consider two
	maps $f,g:A\rightarrow B$.  We say that
	$f$ is \emph{left homotopic} to $g$ ($f\stackrel{l}{\sim}g$) if there
	exists a cylinder object $\tilde{A}$ for $A$
	$$\xymatrix{A\coprod A \ar[r]^-{\nabla} \ar[d]_-{i} & A\\
							\tilde{A} \ar[ur]_-{s}&}
	$$
	together with the following factorization:
	$$\xymatrix{A\coprod A \ar[r]^-{(f,g)} \ar[d]_-{i}& B\\
							\tilde{A} \ar[ur]_-{H}&}
	$$
	The map $H$ is called a \emph{left homotopy} from $f$
	to $g$.
\end{defi}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{defi}
		\label{def.1.1.pathobject}
	Let $\modelcat$ be a model category, and let $X$ be an object of $\modelcat$.
	We say that $\hat{X}$ is a \emph{path object} for $X$, if we have a
	factorization of the diagonal map
	$$\xymatrix{X \ar[r]^-{\Delta} \ar[d]_-{r} & X\times X\\
							\hat{X} \ar[ur]_-{p}&}
	$$
	where $p$ is a fibration and $r$ is a weak equivalence.
\end{defi}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{defi}
		\label{def.1.1.righthomotopy}
	Let $\modelcat$ be a model category and consider two
	maps $f,g:X\rightarrow Y$.  We say that
	$f$ is \emph{right homotopic} to $g$ ($f\stackrel{r}{\sim}$g) if there
	exists a path object $\hat{Y}$ for $Y$
	$$\xymatrix{Y \ar[r]^-{\Delta} \ar[d]_-{r} & Y\times Y\\
							\hat{Y} \ar[ur]_-{p}&}
	$$
	together with the following factorization:
	$$\xymatrix{X \ar[r]^-{(f,g)} \ar[d]_-{H}& Y\times Y\\
							\hat{Y} \ar[ur]_-{p}&}
	$$
	The map $H$ is called a \emph{right homotopy} from $f$
	to $g$.
\end{defi}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{defi}
		\label{def.1.1.homotopymaps}
	Let $\modelcat$ be a model category and consider
	two maps $f,g:A\rightarrow B$.
	We say that $f$ is \emph{homotopic} to $g$ ($f\sim g$) if
	$f$ and $g$ are both left and right homotopic.
\end{defi}

	The following is an elementary but
	extremely useful result.
	
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lem}
		\label{lem.1.1.homot=>symm-wequivs}
	Let $\modelcat$ be a model category, and
	let $f,g:A\rightarrow B$ be two maps in $\modelcat$.
	\begin{enumerate}
		\item	Assume that $f$ and $g$ are left
					homotopic.  Then $f$ is a weak equivalence
					if and only if $g$ is a weak equivalence.
		\item	Assume that $f$ and $g$ are right
					homotopic.  Then $f$ is a weak equivalence
					if and only if $g$ is a weak equivalence.
	\end{enumerate}
\end{lem}
\begin{proof}
	By duality it is enough to prove the first case.
	In this situation, there exists a cylinder object
	$\tilde{A}$ for $A$ together with a left homotopy
	$H:\tilde{A}\rightarrow B$
	between $f$ and $g$  
	$$\xymatrix{A\coprod A \ar[r]^-{(f,g)} \ar[d]_-{i}& B\\
							\tilde{A} \ar[ur]_-{H}&}
	$$
	The following commutative
	diagram and the two out of three property for weak equivalences
	show that $i\iota_{1}$, $i\iota_{2}$ are both
	weak equivalences
	$$\xymatrix{A \ar@<1ex>[r]^-{\iota_{1}} \ar@<-1ex>[r]_-{\iota_{2}}& A\coprod A \ar[r]^-{\nabla} \ar[d]_-{i} & A\\
							&\tilde{A} \ar[ur]_-{s}&}
	$$
	But since $f$ and $g$ are left homotopic we have that
	$f=H(i\iota_{1})$ and $g=H(i\iota_{2})$.
	Therefore $f$ is a weak equivalence if and only if $H$ is a weak equivalence,
	and similarly for $g$.
\end{proof}

	The next result is a corollary of the previous proof.
	
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{cor}
		\label{cor1.1.homotopic=>equal}
	Let $F:\modelcat \rightarrow \mathcal D$ be a functor where $\modelcat$
	is a model category and $F$ maps the class $\mathcal W$ of weak
	equivalences into isomorphisms in $\mathcal D$.
	Let $f,g:A\rightarrow B$ be two maps in $\modelcat$.
	\begin{enumerate}
		\item	If $f$ is left homotopic to $g$, then $F(f)=F(g)$.
		\item	If $f$ is right homotopic to $g$, then $F(f)=F(g)$.
	\end{enumerate}
\end{cor}
\begin{proof}
	By duality we just need to prove the first case.
	We will use the same notation as in the proof of lemma \ref{lem.1.1.homot=>symm-wequivs}.
	We have that $f=H(i\iota _{1})$ and $g=H(i\iota _{2})$, therefore
	it is enough to show that $F(i\iota _{1})=F(i\iota _{2})$.
	But $id_{A}=s(i\iota _{1})=s(i\iota _{2})$ where $s$ is a weak equivalence,
	so $F(s)$ is an isomorphism. We have that $id_{FA}=F(s)F(i\iota _{1})=F(s)F(i\iota _{2})$,
	and cancelling $F(s)$ on the left we get that
	$F(i\iota _{1})=F(i\iota _{2})$.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lem}[cf. \cite{MR0223432}*{I.1 lemma 4}]
		\label{lem.1.1.lefthomotequivrel}
	Let $\modelcat$ be a model category, and let $A$ be a
	cofibrant object in $\modelcat$.  Then for any
	object $B$ in $\modelcat$, the left homotopy
	relation on $\mathrm{Hom}_{\modelcat}(A,B)$ is
	an equivalence relation.
	In this case, $\pi ^{l}_{\modelcat}(A,B)$ will denote
	the set of left homotopy classes of maps between $A$ and $B$.
\end{lem}

	Dually we have:

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lem}
		\label{lem.1.1.righthomotequivrel}
	Let $\modelcat$ be a model category, and let $Y$ be a
	fibrant object in $\modelcat$.  Then for any
	object $X$ in $\modelcat$, the right homotopy
	relation on $\mathrm{Hom}_{\modelcat}(X,Y)$ is
	an equivalence relation.
	In this case, $\pi ^{r}_{\modelcat}(X,Y)$ will denote
	the set of right homotopy classes of maps between $X$ and $Y$.
\end{lem}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lem}[cf. \cite{MR0223432}*{I.1 lemma 5}]
		\label{lem.1.1.left=>right}
	Let $A$ be a cofibrant object in $\modelcat$.
	Suppose that $f,g:A\rightarrow B$ are left homotopic.
	Then given \emph{any} path object $\hat{B}$ for $B$,
	there exists a right homotopy $H:A\rightarrow \hat{B}$
	between $f$ and $g$.
\end{lem}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lem}
		\label{lem.1.1.right=>left}
	Let $Y$ be a fibrant object in $\modelcat$.
	Suppose that $f,g:X\rightarrow Y$ are right homotopic.
	Then given \emph{any} cylinder object $\tilde{A}$ for $A$,
	there exists a left homotopy $H:\tilde{X}\rightarrow Y$
	between $f$ and $g$.
\end{lem}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{cor}
		\label{cor.1.1.homotopy-equiv-rel}
	Let $A,X$ be objects in a model category $\modelcat$, with
	$A$ cofibrant and $X$ fibrant.
	\begin{enumerate}
		\item	The left homotopy, right homotopy, 
					and homotopy relation on $\Hom _{\modelcat}(A,X)$
					are equivalence relations.
		\item	The left homotopy, right homotopy, and homotopy relation
					coincide on $\Hom _{\modelcat}(A,X)$.
	\end{enumerate}
	In this situation, $\pi_{\modelcat}(A,X)$ will denote the \emph{set}
	of homotopy classes of maps between $A$ and $X$.
\end{cor}


	The following is an obvious remark.
	
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{rmk}
		\label{remark1.1.compatibility-one-sided-comp}
	Let $f,g:B\rightarrow C$, $k:C\rightarrow D$
	and $l:A\rightarrow B$ be maps in $\modelcat$.
	\begin{enumerate}
		\item	Suppose that $f$ and $g$ are left homotopic,
					then $kf$ and $kg$ are also left homotopic.
		\item	Suppose that $f$ and $g$ are right homotopic,
					then $fl$ and $gl$ are also right homotopic.
	\end{enumerate}
\end{rmk}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lem}[cf. \cite{MR0223432}*{I.1 lemma 5}]
		\label{lem1.1.fullcompatibility-comp}
	Let $f,g:B\rightarrow C$, $k:C\rightarrow D$, and
	$l:A\rightarrow B$ be maps in $\modelcat$.
	\begin{enumerate}
		\item	Suppose that $B$ is cofibrant, and 
					that $f$ and $g$ are right homotopic,
					then $kf$ and $kg$ are also right homotopic.
		\item	Suppose that $C$ is fibrant, and that
					$f$ and $g$ are left homotopic,
					then $fl$ and $gl$ are also left homotopic.
	\end{enumerate}
\end{lem}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{cor}
		\label{cor.1.1.naivehomotcat}
	Let $\modelcat$ be a model category, and
	let $\modelcat _{cf}$ be the full subcategory
	with objects $X$ such that $X$ is both
	cofibrant and fibrant.
	Then there exists a category
	$\pi \modelcat _{cf}$ with same objects as $\modelcat _{cf}$,
	and where the maps between $X$ and $Y$ are defined as
	the homotopy classes of maps 
	$\pi \modelcat _{cf}(X,Y)=\pi_{\modelcat}(X,Y)$ between $X$ and $Y$
	in $\modelcat$.  The compositon law in $\pi \modelcat _{cf}$ is
	induced from the one in $\modelcat _{cf}$. 
\end{cor}
\begin{proof}
	Follows immediately from corollary \ref{cor.1.1.homotopy-equiv-rel}
	and lemma \ref{lem1.1.fullcompatibility-comp}.
\end{proof}

	The category $\pi \modelcat _{cf}$ will be called
	the \emph{naive homotopy category} of $\modelcat$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lem}[cf. \cite{MR0223432}*{I.1 lemma 7}]
		\label{lem1.1.trivfib=>iso-on=homgrps}
	Let $\modelcat$ be a model category, and let
	$f:X\rightarrow Y$ be a trivial cofibration.
	Then for every cofibrant object $A$, we get
	an isomorphism $f_{*}:\pi^{l}(A,X)\rightarrow \pi^{l}(A,Y)$.
\end{lem}
\begin{proof}
	Let $[g]\in \pi^{l}(A,Y)$ be an arbitrary element, which
	is represented by a map $g:A\rightarrow Y$ between $A$
	and $Y$.  Since $f$ is a trivial fibration, the lifting axiom $\mathbf{MC4}$
	implies that there exists a map $s$ making the next diagram commutative
	$$\xymatrix{\emptyset \ar[r] \ar[d]& X \ar[d]^-{f}\\
							A \ar[r]_-{g} \ar@{-->}[ur]^-{s}& Y}
	$$
	this shows the surjectivity of $f_{*}$.
	Now suppose $k,l:A\rightarrow X$ are two maps such that
	$pk\stackrel{l}{\sim}pl$.  Let $H:\tilde{A}\rightarrow Y$
	be a left homotopy between $pk$ and $pl$.
	Then since $p$ is a trivial fibration, the lifting axiom $\mathbf{MC4}$
	implies that there exists an arrow $G$ making the following diagram
	commutative
	$$\xymatrix{A\coprod A \ar[r]^-{(f,g)} \ar[d]_-{i}& X \ar[d]^-{p}\\
							\tilde{A} \ar[r]_-{H} \ar@{-->}[ur]^-{G}& Y}
	$$
	therefore $k\stackrel{l}{\sim}l$, and this shows the injectivity
	of $f_{*}$.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{cor}[cf. \cite{MR0223432}*{I.1 lemma 7}, 
							\cite{MR1650134}*{proposition 1.2.5}]
		\label{cor1.1.weakequiv=>isosin-Homot}
	Let $\modelcat$ be a model category and consider a map
	$f:X\rightarrow Y$.
	\begin{enumerate}
		\item	Assume that $X$ and $Y$ are both cofibrant.  If
					$f$ is a weak equivalence then for every fibrant
					object $Z$ in $\modelcat$, the induced map
					$f^{*}:\pi_{\modelcat}(Y,Z)\rightarrow \pi_{\modelcat}(X,Z)$
					is a bijection.
		\item	Assume that $X$ and $Y$ are both fibrant.  If $f$ is a weak equivalence
					then for every cofibrant object $A$ in $\modelcat$, the induced
					map $f_{*}:\pi_{\modelcat}(A,X)\rightarrow \pi_{\modelcat}(A,Y)$
					is a bijection. 
	\end{enumerate}
\end{cor}
\begin{proof}
		By duality it is enough to prove only the first case.
		Assume that $f$ is a weak equivalence between cofibrant objects.
		Since bijections of sets clearly satisfy the two out of three property,
		Ken Brown's lemma (see lemma \ref{lem1.1.KenBrown}) implies that it is
		enough to consider the case in which $f$ is a trivial cofibration.
		Let $[k]$ be an arbitrary element of $\pi_{\modelcat}(X,Z)$, then
		since we are assuming that $f$ is a trivial cofibration and $Z$ is a fibrant object,
		the lifting axiom $\mathbf{MC4}$ implies that
		the dotted arrow making the following diagram commutative exists
		$$\xymatrix{X \ar[r]^-{k} \ar[d]_-{f}& Z \ar[d]\\
								Y \ar[r] \ar@{-->}[ur]^-{s}& \ast}
		$$
		and this gives the surjectivity of $f^{*}$.
		Now assume that $k,l:Y\rightarrow Z$ are two maps in $\modelcat$ such
		that $kf,lf:X\rightarrow Z$ are homotopic.
		Since $X$ is cofibrant and $Z$ is fibrant we can assume
		that $kf$ and $lf$ are right homotopic, 
		$$\xymatrix{X \ar[rr]^-{(kf,lf)} \ar[d]_-{H} && Z\times Z \\
								\hat{Z} \ar[urr]_-{p}&&}
		$$
		Then since $p$ is a fibration by definition, axiom $\mathbf{MC4}$ gives a map $K$
		making the following diagram commutative:
		$$\xymatrix{X \ar[r]^-{H} \ar[d]_-{f}& \hat{Z} \ar[d]^-{p}\\
								Y \ar[r]_-{(k,l)} \ar@{-->}[ur]^-{K}& Z\times Z}
		$$
		This shows that $k$ and $l$ are also homotopic, and therefore
		we have the injectivity of $f^{*}$.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{thm}[Whitehead's theorem for model categories]
		\label{thm.1.1.Weak-Whitehead's-thm}
	Let $\modelcat$ be a model category, and
	consider two cofibrant and fibrant objects
	$X,Y$ of $\modelcat$.
	Then $f:X\rightarrow Y$ is a weak equivalence
	if and only if it is a homotopy equivalence.
\end{thm}
\begin{proof}
	Suppose that $f$ is a weak equivalence.
	Since $X,Y$ are cofibrant and fibrant, corollary \ref{cor1.1.weakequiv=>isosin-Homot}
	implies that $f^{*}:\pi_{\modelcat}(Y,X)\rightarrow \pi_{\modelcat}(X,X)$ is
	a bijection.  In particular there exists $g:Y\rightarrow X$ such that
	$gf\sim id_{X}$.  Similarly we have that
	$f^{*}:\pi_{\modelcat}(Y,Y)\rightarrow \pi_{\modelcat}(X,Y)$ is a bijection.
	But $[id_{Y}]\mapsto [f]$ and $[fg]\mapsto [fgf]=[f]$ (since $gf\sim id_{X}$),
	so the injectivity of $f^{*}$ shows that $fg$ is homotopic to $id_{Y}$.
	Thus $f$ is a homotopy equivalence.
	
	Conversely, assume that $f$ is a homotopy equivalence with homotopy
	inverse $g$.
	Factor $f$ as
	$$\xymatrix{X \ar[r]^-{i}& Z \ar[r]^-{m}& Y}
	$$
	where $m$ is a trivial fibration and
	$i$ is a cofibration.  It is enough to show that $i$ is
	a weak equivalence.
	The previous argument shows
	that $m$ is a homotopy equivalence, let $n$ be a homotopy inverse
	for $m$.  We have that $gf\sim id_{X}$, i.e. $gmi\sim id_{X}$.
	Let $H$ be a right homotopy between $gmi$ and $id_{X}$:
	$$\xymatrix{X \ar[rr]^-{(gmi,id_{X})} \ar[d]_-{H} && X\times X\\
							\hat{X} \ar[urr]_-{p}&&}
	$$
	Since $X$ is fibrant, the following commutative diagram shows
	$$\xymatrix{X \ar[r]^-{\Delta} \ar[d]_-{s} & X\times X \ar[r]^-{\pi_{2}} \ar[d]^-{\pi_{1}}& X \ar[d]\\
							\hat{X}\ar[ur]_-{p}& X \ar[r]& \ast}
	$$
	that the maps $\pi_{1}p$, $\pi_{2}p$ are both trivial fibrations.
	The lifting axiom $\mathbf{MC4}$ implies that there exists a map $K$
	making the following diagram commutative
	$$\xymatrix{X \ar[r]^-{H} \ar[d]_-{i}& \hat{X} \ar[d]^-{\pi_{1}p}\\
							Z \ar[r]_-{gm} \ar@{-->}[ur]^-{K}& X}
	$$
	Let $q=\pi_{2}pK$, then $qi=id_{X}$ and $q\sim gm$.
	The following diagram shows that $i$ is a retract of $iq$:
	$$\xymatrix{X \ar[r]^-{i} \ar[d]_-{i}& Z \ar[r]^-{q} \ar[d]^-{iq}& X \ar[d]^-{i}\\
							Z \ar[r]_{id}& Z \ar[r]_-{id}& Z}
	$$
	therefore it is enough to show that $iq$ is a weak equivalence.
	But we have that $iq \sim nmiq \sim nfq \sim nfgm \sim nm \sim id_{Z}$.
	So lemma \ref{lem.1.1.homot=>symm-wequivs} implies that $iq$ is a weak equivalence.
\end{proof}		
		

%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{defi}[cf. \cite{MR0223432}*{I.1 definition 5}]
		\label{def.1.2.loc-of-cats}
	Let $\modelcat$ be an arbitrary category and
	$\mathcal W$ a class of maps in $\modelcat$.
	The \emph{localization} of
	$\modelcat$ with respect to $\mathcal W$
	will be a category $\mathcal W ^{-1}\modelcat$
	together with a functor $\gamma :\modelcat \rightarrow \mathcal W ^{-1}\modelcat$
	having the following universal property:
	for every $w\in \mathcal W$, $\gamma (w)$ is an isomorphism, and
	given any functor $F:\modelcat \rightarrow \mathcal D$ such that
	$F(w)$ is an isomorphism for every $w\in \mathcal W$, there is a unique
	functor $\theta :\mathcal W ^{-1}\modelcat \rightarrow \mathcal D$,
	such that $\theta \circ \gamma =F$, i.e. the following
	diagram commutes:
	$$\xymatrix{\modelcat \ar[r]^-{F} \ar[d]_-{\gamma}& \mathcal D\\
							\mathcal W ^{-1}\modelcat \ar@{-->}[ur]_-{\theta}&}
	$$
\end{defi}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{thm}[cf. \cite{MR0223432}*{I.1 theorem 1}]
		\label{thm.1.1.HomotCat-exist}
	Let $\modelcat$ be a model category.
	Then there exists a category $\hocat$, which is the localization
	of $\modelcat$ with respect to the class $\mathcal W$ of weak equivalences,
	and is called the \emph{homotopy category}
	of $\modelcat$.  $\hocat$ is
	defined as follows:
	\begin{enumerate}
		\item	The objects of $\hocat$ are
					just the objects in $\modelcat$.
		\item	The set of maps in $\hocat$ between two
					objects $X,Y$ is given by
					the set of homotopy classes between
					cofibrant-fibrant replacements for
					$X$ and $Y$:
					$$\Hom_{\hocat}(X,Y)=\Hom_{\pi \modelcat_{cf}}(RQX,RQY)=\pi_{\modelcat}(RQX,RQY)$$
					and the composition law is induced by the composition
					in $\pi \modelcat _{cf}$ (see corollary \ref{cor.1.1.naivehomotcat}).
	\end{enumerate}
	Let $\hocat _{c}$, $\hocat _{f}$, $\hocat _{cf}$ be the full
	subcategories of $\hocat$ generated by the cofibrant, fibrant
	and cofibrant-fibrant objects of $\modelcat$ respectively.
	In the following diagram, all the functors are equivalences of
	categories:
	$$\xymatrix{&&& \hocat_{c} \ar@<-1ex>@{_{(}->}[drr]_-{\sim} \ar@<1ex>[lld]^-{\mathrm{Ho}R}&& \\
							\pi \modelcat_{cf} \ar[r]^-{\sim} & \hocat_{cf} 
							\ar@<1ex>@{^{(}->}[urr]^-{\sim} \ar@<-1ex>@{_{(}->}[drr]_-{\sim} &&&& 
							\hocat \ar@<-1ex>[llu]_-{\mathrm{Ho}Q} \ar@<1ex>[dll]^-{\mathrm{Ho}R}\\
							&&& \hocat_{f} \ar@<1ex>@{^{(}->}[urr]^-{\sim} \ar@<-1ex>[ull]_-{\mathrm{Ho}Q}&&}
	$$
	where the adjoints to the equivalences given above are constructed
	taking cofibrant, fibrant and cofibrant-fibrant replacements.
\end{thm}
\begin{proof}
	We refer the reader to \cite{MR0223432}*{I.1 theorem 1}.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{cor}
		\label{cor1.2.Hom-in-hocat}
	Let $\modelcat$ be a model category, and consider
	a pair of objects $A,X$ in $\modelcat$, where $A$ is cofibrant
	and $X$ is fibrant.  Then there is a natural isomorphism
	$\Hom _{\hocat}(A,X)\cong \pi _{\modelcat}(A,X)$.
\end{cor}
\begin{proof}
	We have that $\Hom _{\hocat}(A,X)=\pi _{\modelcat}(RQA,RQX)$.
	Since $A$ is cofibrant and $X$ is fibrant we can apply
	corollary \ref{cor1.1.weakequiv=>isosin-Homot} to get
	the following natural isomorphisms:
	\begin{eqnarray*}
	  \pi _{\modelcat}(RQA,RQX) &\cong &
		\pi _{\modelcat}(QA,RQX) \cong  \pi _{\modelcat}(QA,QX)\\
		&\cong & \pi _{\modelcat} (A,QX) \cong  \pi _{\modelcat}(A,X)
	\end{eqnarray*}
	this completes the proof.
\end{proof}

\end{section}

==> chapters/sections-1/subsect-1.2/subsect-leftBousloc.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{section}{Left Bousfield Localization}
		\label{subsection.LeftBousfieldLocalization}
	In this section we show the existence of the left
	Bousfield localization for a model category $\modelcat$ which satisfies
	certain conditions (\emph{cellularity and left properness})
	with respect to a \emph{set}
	$\mathcal V$ of maps.
	
	The main result is the following:

%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{thm}[Hirschhorn, \cite{MR1944041}*{theorem 4.1.1}]
		\label{thm1.2.2.Existence-leftBous}
	Let $\modelcat$ be a left proper cellular model category
	and let $\mathcal V$ be a \emph{set} of maps in $\modelcat$.
	\begin{enumerate}
		\item	\label{thm1.2.2.Existence-leftBous.a}	The left Bousfield localization $\leftBousloc$
					of $\modelcat$ with respect to $\mathcal V$ exists
					(see definition \ref{def1.2.1.leftBousloc}).
		\item	\label{thm1.2.2.Existence-leftBous.b} The fibrant objects of $\leftBousloc$
					are the \local objects of $\modelcat$ (see definition \ref{def1.2localob-weq}).
		\item	\label{thm1.2.2.Existence-leftBous.c}	$\leftBousloc$ is a left proper cellular	
					model category, where the set of generating cofibrations $I$ is equal to the one in $\modelcat$,
					and the set of generating trivial cofibrations $J_{\mathcal V}$ is the one
					given by theorem \ref{thm1.2.2.existence-trivcof-gen}.
		\item	\label{thm1.2.2.Existence-leftBous.d}	$\leftBousloc$ is a simplicial model category
					with simplicial structure induced from the one in $\modelcat$
					(we are assuming that all our model categories $\modelcat$ are simplicial).
		\end{enumerate}
\end{thm}
	
	
%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{defi}
		\label{def.1.2.2.Horns-on-S}
	If $\modelcat$ is a model category and $\mathcal V$ is a class of maps
	in $\modelcat$, then a \emph{full class of horns on}
	$\mathcal V$ is a class $\Lambda (\mathcal V )$ of maps obtained
	by choosing for every element $i:A\rightarrow B$ of $\mathcal V$
	a horn $\Lambda _{i}$ (see definition \ref{def.1.2.1.horn}), and letting
	$\Lambda (\mathcal V )$ be the class of maps
	$$\Lambda (\mathcal V )=\{ \Lambda _{i} | (i:A\rightarrow B)\in \mathcal V \}
	$$
\end{defi}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{defi}
		\label{def.1.2.2.augmented-Horns}
	Let $\modelcat$ be a cofibrantly generated model category
	(see definition \ref{def1.2.cofgen}) with generating cofibrations
	$I$ and generating trivial cofibrations $J$.  If
	$\mathcal V$ is a \emph{set} of maps of $\modelcat$,
	then an \emph{augmented set of $\mathcal V$-horns} is a \emph{set}
	$\overline{\Lambda (\mathcal V )}$ of maps
	$$\overline{\Lambda(\mathcal V )}=\Lambda (\mathcal V ) \cup J
	$$
	for some full set of horns $\Lambda (\mathcal V )$ on $\mathcal V$
	(see definition \ref{def.1.2.2.Horns-on-S}).
\end{defi}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{prop}[cf. \cite{MR1944041}*{proposition 4.2.3}]
		\label{prop1.2.2.aughorns=>loceq}
	If $\modelcat$ is a left proper cellular model category and
	$\mathcal V$ is a \emph{set} of maps in $\modelcat$,
	then every element of an augmented set of horns on $\mathcal V$
	is a \local equivalence.
\end{prop}
\begin{proof}
	We need to show that every element of
	$\overline{\Lambda (\mathcal V )}=\Lambda (\mathcal V )\cup J$ is a \local equivalence.
	That the maps in $J$ are \local equivalences follows from proposition
	\ref{prop1.2.weq-are-local}.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{prop}[cf. \cite{MR1944041}*{proposition 4.2.4}]
		\label{prop1.2.2.class-loc-obj}
	Let $\modelcat$ be a left proper and cellular model category and
	$\mathcal V$ a \emph{set} of maps in $\modelcat$.
	An object $X$ of $\modelcat$
	is \local if and only if the map $X\rightarrow *$ has the
	right lifting property with
	respect to an augmented set of horns.
\end{prop}
\begin{proof}
	Follows immediately from lemma \ref{lem1.2.1.class-loc-obj}
	and the fact that fibrant objects $X$ are characterized by
	the right lifting property of $X\rightarrow *$ with respect
	to the generating trivial cofibrations $J$.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{prop}[cf. \cite{MR1944041}*{proposition 4.2.5}]
		\label{prop1.2.1.cells-wrt-aug-horns}
	Let $\modelcat$ be a left proper cellular model category with set of generating
	cofibrations $I$ and let $\mathcal V$ be a \emph{set} of maps in $\modelcat$.
	Then there exists a \emph{set} $\widetilde{\Lambda (\mathcal V )}$
	of relative $I$-cell complexes with cofibrant domains such that
	the following conditions are satisfied:
	\begin{enumerate}
		\item	\label{prop1.2.1.cells-wrt-aug-horns.a}	Every map in
					$\widetilde{\Lambda (\mathcal V )}$ is a \local equivalence.
		\item	\label{prop1.2.1.cells-wrt-aug-horns.b}	An object $X$ in $\modelcat$
					is \local if and only if the map $X\rightarrow *$ is
					$\widetilde{\Lambda (\mathcal V )}$-injective.
	\end{enumerate}
\end{prop}
\begin{proof}
	Choose a full set of horns on $\mathcal V$.  For any map
	$i:A\rightarrow B$ in $\Lambda (\mathcal V )$, apply Quillen's small
	object argument to get a factorization as 
	$\xymatrix{A \ar[r]^-{\tilde{\imath}} & C \ar[r]^-{p} & B}$ where
	$\tilde{\imath}$ is a relative $I$-cell complex and $p$ is a trivial fibration.
	By remark \ref{horns-cohorns-cof-fib} we know that $i:A\rightarrow B$
	is a cofibration, i.e. $i$ has the left lifting property with respect
	to $p$.  Then the retract argument (see proposition \ref{prop1.1.retract})
	implies that $i$ is a retract of $\tilde{\imath}$.
	Since $p$ and $i$ are \local equivalences, the two out of three property
	for \local equivalences implies that $\tilde{\imath}$ is
	a \local-equivalence.
	
	We also have the following general fact about cofibrantly generated model
	categories: there is a \emph{set} $\tilde{J}$ of generating
	trivial cofibrations for $\modelcat$ such that every element of
	$\tilde{J}$ is a relative $I$-cell complex with cofibrant domain.
	We take
	$$\widetilde{S}=\tilde{J}\cup \{ \tilde{\imath}|i\in \Lambda (\mathcal V )\}
	$$
	To finish the proof we only need to check that condition \ref{prop1.2.1.cells-wrt-aug-horns.b}
	holds.  But this follows immediately from proposition \ref{prop1.2.2.class-loc-obj},
	and the fact that lifting properties are preserved under retracts.
	
	%Suppose that $X\rightarrow *$ is $\widetilde{\Lambda (\mathcal V )}$-injective,
	%then lemma \ref{lem1.2.1.class-loc-obj}
	%together with the fact that right and left lifting properties are preserved under retracts,
	%imply that $X$ is \local.  Conversely, if $X$ is \local, then $X$ is fibrant so 
	%in particular $X\rightarrow *$ has the right lifting property with repect to $\tilde{J}$,
	%on the other hand lemma \ref{lem1.2.1.class-loc-obj} implies that $X$ has the
	%right lifting property with respect to $\{ \tilde{i}|i\in \Lambda (\mathcal V ) \}$.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{cor}[cf. \cite{MR1944041}*{proposition 4.2.7}]
		\label{cor1.12.V-cell-complexes-inj}
	Let $\modelcat$ be a left proper cellular model category, and let
	$\mathcal V$ be a set of maps in $\modelcat$.  An object
	$X$ of $\modelcat$ is \local if and only if
	$X\rightarrow *$ has the right lifting property with respect to
	all relative $\widetilde{\Lambda (\mathcal V )}$-cell complexes.
\end{cor}
\begin{proof}
	Follows immediately from proposition \ref{prop1.2.1.cells-wrt-aug-horns}, and
	the fact that the left lifting property is preserved under pushouts
	and $\lambda$-sequences.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{thm}[cf. \cite{MR1944041}*{theorem 4.2.9}]
		\label{thm1.2.2.relcompl=>cof-we}
	Let $\modelcat$ be a left proper cellular model category and let $\mathcal V$
	be a \emph{set} of objects in $\modelcat$.  Then every relative
	$\widetilde{\Lambda (\mathcal V )}$-cell complex is 
	a cofibration and a \local equivalence.
\end{thm}
\begin{proof}
	Follows immediately from propositions \ref{prop1.2.pushoutloceq}
	and \ref{prop1.2.trancomploceq}.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{prop}[cf. \cite{MR1944041}*{proposition 4.2.10}]
		\label{prop1.2.2.relcells-loc}
	Let $\modelcat$ be a left proper cellular model category, and let
	$\mathcal V$ be a set of maps in $\modelcat$.  If $j:X\rightarrow \hat{X}$
	is a relative $\widetilde{\Lambda (\mathcal V )}$-cell complex and
	$\hat{X}$ is a $\widetilde{\Lambda (\mathcal V )}$-injective, then
	$(\hat{X},j)$ is a cofibrant $\mathcal V$-localization of $X$.
\end{prop}
\begin{proof}
	Follows immediately from theorem \ref{thm1.2.2.relcompl=>cof-we}
	and proposition \ref{prop1.2.1.cells-wrt-aug-horns}.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{thm}[cf. \cite{MR1944041}*{theorem 4.3.8}]
		\label{thm1.2.2.simplocfunctor}
	Let $\modelcat$ be a left proper cellular model category and
	let $\mathcal V$ be a \emph{set} of maps in $\modelcat$.  Then
	for any map $X\rightarrow Y$ in $\mathcal M$
	there exists a natural factorization 
	$$\xymatrix{X \ar[r]^-{j}& L_{\mathcal V}\ar[r]^-{p}& Y}
	$$
	where $j$ is a relative $\widetilde{\Lambda (\mathcal V )}$-cell
	complex and $p$ is $\widetilde{\Lambda (\mathcal V )}$-injective.
	Furthermore, this factorization is a simplicial functor.
\end{thm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{defi}
		\label{def1.2.2.simplocfunctor}
	Let $\modelcat$ be a left proper cellular model category, and let
	$\mathcal V$ be a \emph{set} of maps in $\modelcat$.  The
	\emph{$\mathcal V$-localization} of an object $X$ is the
	object $L_{\mathcal V}X$ obtained by applying the factorization
	of theorem \ref{thm1.2.2.simplocfunctor} to the map $X\rightarrow *$.
	This factorization defines a natural transformation
	$j:id\rightarrow L_{\mathcal V}$ such that $j(X):X\rightarrow L_{\mathcal V}X$ is
	a relative $\widetilde{\Lambda (\mathcal V )}$-cell complex for every
	object $X$.
\end{defi}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{thm}[cf. \cite{MR1944041}*{theorem 4.3.3}]
		\label{thm1.2.2.simplocfunctor=>cof-loc}
	Let $\modelcat$ be a left proper cellular model category and
	let $\mathcal V$ be a \emph{set} of maps in $\modelcat$.
	Then for every object $X$ in $\modelcat$, the $\mathcal V$-localization
	$j(X):X\rightarrow L_{\mathcal V}X$ is a cofibrant
	$\mathcal V$-localization of $X$.
\end{thm}
\begin{proof}
	Follows immediately from proposition \ref{prop1.2.2.relcells-loc}.
\end{proof}

	We then get the following corollary:
	
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{cor}[cf. \cite{MR1944041}*{corollary 4.3.4}]
		\label{cor1.2.2.existence-loc}
	Let $\modelcat$ be a left proper cellular model category and
	let $\mathcal V$ be a \emph{set} of maps in $\modelcat$.
	Then every object has a $\mathcal V$-localization.
\end{cor}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{thm}[cf. \cite{MR1944041}*{theorem 4.3.5}]
		\label{thm1.2.2.class-loc-obj}
	Let $\modelcat$ be a left proper cellular model category, and let
	$\mathcal V$ be a \emph{set} of maps in $\modelcat$.
	If $X$ is a fibrant object, then $X$ is \local if and only if
	the $\mathcal V$-localization map $j(X):X\rightarrow L_{\mathcal V}X$
	is a weak equivalence.
\end{thm}
\begin{proof}
	Follows immediately from theorem \ref{thm1.2.co-loc-detect}.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{thm}[cf. \cite{MR1944041}*{theorem 4.3.6}]
		\label{thm1.2.2.class-loc-we}
	Let $\modelcat$ be a left proper cellular model category, and let
	$\mathcal V$ be a \emph{set} of maps in $\modelcat$.  The map
	$f:X\rightarrow Y$ is a \local equivalence if and only if
	its $\mathcal V$-localization
	$L_{\mathcal V}(f):L_{\mathcal V}X\rightarrow L_{\mathcal V}Y$
	is a weak equivalence.
\end{thm}
\begin{proof}
	Follows immediately from theorem \ref{thm1.2.co-locequiv-detect}.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{prop}[cf. \cite{MR1944041}*{proposition 4.4.1}]
	Let $\modelcat$ be a left proper cellular model category,
	and let $\mathcal V$ be a \emph{set} of maps in $\modelcat$.
	If $i:A\rightarrow B$ is the inclusion of a subcomplex,
	then so is $L_{\mathcal V}(i):L_{\mathcal V}A\rightarrow L_{\mathcal V}B$.
\end{prop}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{prop}[cf. \cite{MR1944041}*{proposition 4.4.3}]
	Let $\modelcat$ be a left proper cellular model category and let
	$\mathcal V$ be a \emph{set} of maps in $\modelcat$.
	If $i:A\rightarrow B$ is the inclusion of a subcomplex,
	then $i$ is a \local equivalence if and only if its
	localization $L_{\mathcal V}(i):L_{\mathcal V}A\rightarrow L_{\mathcal V}B$
	is the inclusion of a strong deformation retract.
\end{prop}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{prop}[cf. \cite{MR1944041}*{proposition 4.4.4}]
	Let $\modelcat$ be a left proper cellular model category and let
	$\mathcal V$ be a \emph{set} of maps in $\modelcat$.
	If $X$ is a cell complex and
	$K_{0}\subset K_{1}\subset \cdots \subset K_{\beta}\subset \cdots$
	($\beta <\lambda$) is a $\lambda$-sequence of subcomplexes of
	$X$ (where $\lambda$ is the ordinal chosen in the proof of theorem \ref{thm1.2.2.simplocfunctor}),
	then the natural map
	$\mathrm{colim}_{\beta <\lambda}L_{\mathcal V}K_{\beta}\rightarrow L_{\mathcal V}(\mathrm{colim}_{\beta <\lambda}K_{\beta})$
	is an isomorphism.
\end{prop}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{prop}[cf. \cite{MR1944041}*{proposition 4.4.5}]
	Let $\modelcat$ be a left proper cellular model category and let $\mathcal V$
	be a \emph{set} of maps in $\modelcat$.  If $C$ is a cell complex and
	$A$ and $B$ are subcomplexes of $C$, then the natural map
	$L_{\mathcal V}(A\cap B)\rightarrow (L_{\mathcal V}A)\cap (L_{\mathcal V}B)$
	is an isomorphism.
\end{prop}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{thm}[cf. \cite{MR1944041}*{proposition 4.5.1}]
		\label{thm1.2.2.existence-trivcof-gen}
	If $\modelcat$ is a left proper cellular model category and $\mathcal V$
	is a \emph{set} of maps in $\modelcat$, then there is a set
	$J_{\mathcal V}$ of inclusions of cell complexes such that the
	class of $J_{\mathcal V}$-cofibrations equals the class of cofibrations
	that are also \local equivalences.
\end{thm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lem}[cf. \cite{MR1944041}*{lemma 4.5.2}]
		\label{lem1.12.properness=>cellcplxs}
	Let $\modelcat$ be a left proper cellular model category and
	let $\mathcal V$ be a set of maps in $\modelcat$.
	If $p:X\rightarrow Y$ is a fibration with the right lifting property
	with respect to all inclusions of cell complexes that are
	\local equivalences, then it has the right lifting property
	with respect to all cofibrations that are \local equivalences.
\end{lem}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{defi}
		\label{def1.12.size-of-localization}
	Let $\modelcat$ be a left proper cellular model category and
	let $\mathcal V$ be a set of maps in $\modelcat$, we let
	$\xi$ be the smallest cardinal that is at least as large
	as each of the following cardinals:
	\begin{enumerate}
		\item	The size of the cells of $\modelcat$
					(see definition \ref{def.1.1.2.size-M}).
		\item	A cardinal $\eta$ such that the domain of every
					map in $I$ is $\eta$-compact.
		\item	The cardinal $\lambda$ selected in the proof
					of theorem \ref{thm1.2.2.simplocfunctor}.
		\item	The cardinal $\kappa$ described in \cite{MR1944041}*{proposition 12.5.3}
					for the set $\widetilde{\Lambda (\mathcal V)}$.
		\item	The cardinal $\kappa$ described in \cite{MR1944041}*{proposition 12.5.7}
	\end{enumerate}
	and we let $\gamma$ denote the cardinal $\gamma =\xi ^{\xi}$.
\end{defi}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lem}[cf. \cite{MR1944041}*{lemma 4.5.4}]
		\label{lem.1.12.cardinal-bounding-complxs}
	Let $\modelcat$ be a left proper cellular model category and
	let $\mathcal V$ be a \emph{set} of maps in $\modelcat$.
	If $A$ is a cell complex of size at most $\gamma$
	(see definition \ref{def1.2.1.size-cell-complex}),
	then $L_{\mathcal V}A$ has size at most $\gamma$.
\end{lem}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{prop}[cf. \cite{MR1944041}*{proposition 4.5.5}]
		\label{prop1.12.subcplxs-generate}
	Let $\modelcat$ be a left proper cellular model category,
	let $\mathcal V$ be a set of maps in $\modelcat$, and let
	$B$ be a cell complex.  If $i:A\rightarrow B$ is the inclusion
	of a proper subcomplex and a \local equivalence, then
	there exists a subcomplex $C$ of $B$ such that:
	\begin{enumerate}
		\item	The subcomplex $C$ is not contained in the subcomplex $A$.
		\item	The size of $C$ is at most $\gamma$.
		\item	The inclusions $A\cap C\rightarrow C$ and
					$A\rightarrow A\cup C$ are both \local equivalences.
	\end{enumerate}
\end{prop}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{prop}[cf. \cite{MR1944041}*{proposition 4.5.6}]
		\label{prop.1.12.triv-cof-gen-leftBousloc}
	Let $\modelcat$ be a left proper cellular model category and
	let $\mathcal V$ be a set of maps in $\modelcat$.
	If $p:X\rightarrow Y$ has the right lifting property with
	respect to those inclusions of subcomplexes $i:A\rightarrow B$
	that are \local equivalences and such that the size of $B$ is
	at most $\gamma$ (see definition \ref{def1.12.size-of-localization}),
	then $p$ has the right lifting property with
	respect to all inclusions of subcomplexes that are
	\local equivalences.
\end{prop}

\end{section}


==> chapters/sections-1/subsect-1.2/subsect-rightBousloc.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{section}{Right Bousfield Localization}
		\label{subsection-rightBousloc}
		
	In this section we show the existence of the
	right Bousfield localization under certain
	conditions (\emph{cellularity and right properness}) which
	are dual to the ones for left Bousfield localization.
	However, it is not possible to prove in general that
	the model structure for the right Bousfield localization
	is cofibrantly generated.  The main existence theorem is the
	following:

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{thm}
		\label{thm1.2.3.existence-rightBousloc}
	Let $\modelcat$ be a right proper cellular model category, let
	$K$ be a \emph{set} of objects in $\modelcat$, and let
	$\mathcal V$ be the class of $K$-colocal equivalences
	(see definition \ref{def1.2.cellularization}).
	\begin{enumerate}
		\item	\label{thm1.2.3.existence-rightBousloc.a}	The right Bousfield localization of $\modelcat$
					with respect to $\mathcal V$ exists (see definition \ref{def1.2.1.rightBousloc}).
		\item	\label{thm1.2.3.existence-rightBousloc.b}	The cofibrant objects
					of $\rightBousloc$ are the \colocal objects of $\modelcat$.
		\item	\label{thm1.2.3.existence-rightBousloc.c}	$\rightBousloc$ is a
					right proper model category.
		\item	\label{thm1.2.3.existence-rightBousloc.d}	$\rightBousloc$ is a simplicial model
					category, with simplicial structure induced from the one existing in
					$\modelcat$.
	\end{enumerate}
\end{thm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{defi}
		\label{def1.2.3.K-colocal-cofs}
	Let $\modelcat$ be a model category, and $K$ a \emph{set}
	of objects in $\modelcat$.  A map
	$i:A\rightarrow B$ in $\modelcat$ is called a \emph{$K$-colocal
	cofibration} if it has the left lifting property with respect to the class
	of maps which are both fibrations in $\modelcat$ and $K$-colocal equivalences.
\end{defi}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{defi}
		\label{def1.2.3.horns-onK}
	Let $\modelcat$ be a right proper cellular model category with
	generating cofibrations $I$ and generating trivial cofibrations $J$,
	and let $K$ be a \emph{set} of objects of $\modelcat$.
	\begin{enumerate}
		\item	\label{def1.2.3.horns-onK.a}	A \emph{full set of horns on}
					$K$ is a set $\Lambda (K)$ of maps obtained by choosing
					a cofibrant resolution $QA$ of every element $A$ in $K$ and letting
					$$\Lambda (K)=\{ QA\otimes \partial \Delta ^{n}\rightarrow QA\otimes \Delta ^{n}|n\geq 0\}
					$$
		\item	\label{def1.2.3.horns-onK.b}	An \emph{augmented set of $K$-horns} is a set
					$\overline{\Lambda (K)}$ of maps
					$$\overline{\Lambda (K)}=\Lambda (K)\cup J
					$$
					for some full set of horns $\Lambda (K)$ on $K$.
	\end{enumerate}
\end{defi}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{prop}
		\label{prop1.2.3.Kcomplex-factor}
	Let $\modelcat$ be a right proper cellular model category.  If $K$
	is a set of objects of $\modelcat$, then there is a functorial factorization
	of every map $j:A\rightarrow B$ as
	$\xymatrix{A \ar[r]^-{i}& C \ar[r]^-{q}& B}$
	where $i$ is a relative $\overline{\Lambda (K)}$-cell complex and
	$q$ is a $\overline{\Lambda (K)}$-injective.
\end{prop}
\begin{proof}
	This is just an application of Quillen's small object argument.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{prop}
		\label{prop1.2.3.class-inj}
	Let $\modelcat$ be a right proper cellular model category and let $K$
	be a \emph{set} of objects of $\modelcat$.  If $Y$ is a fibrant object
	of $\modelcat$, then a map $q:X\rightarrow Y$ is a $\overline{\Lambda (K)}$-injective
	if and only if it is both a fibration and a $K$-colocal equivalence.
\end{prop}
\begin{proof}
	Since $\modelcat$ is cofibrantly generated, $q$ is a fibration if and only if
	it is $J$-injective.  Assume that $q$ is a fibration, then $X$ is also
	fibrant, and then $q$ is already a fibrant resolution, then
	a simplicial adjunction argument shows that $q$ is $\overline{\Lambda (K)}$-injective
	if and only if $q$ is a $K$-colocal equivalence.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{prop}
		\label{prop1.2.3.cellcomplex=>coloc-cof}
	Let $\modelcat$ be a right proper cellular model category.
	If $K$ is a set of objects of $\modelcat$, then a relative
	$\overline{\Lambda (K)}$-cell complex is a $K$-colocal
	cofibration (see definition \ref{def1.2.3.K-colocal-cofs}).
\end{prop}
\begin{proof}
	Let $q:X\rightarrow Y$ be a fibration and a $K$-colocal equivalence,
	and let $i:A\rightarrow B$ be a relative $\overline{\Lambda (K)}$-cell complex.
	Then we must find a lifting in every solid commutative diagram
	$$\xymatrix{A \ar[r] \ar[d]_-{i}& X \ar[d]^-{q}\\
							B \ar[r] \ar@{-->}[ur]^{s}& Y}
	$$
	Since $\modelcat$ is right proper, it is enough to find the lifting
	for a fibrant approximation $\hat{q}$ of $q$ where
	$\hat{q}$ is a fibration and a $K$-colocal equivalence.  But proposition \ref{prop1.2.3.class-inj}
	implies that $\hat{q}$ is $\overline{\Lambda (K)}$-injective,
	so the required lifting exists.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lem}
		\label{lem1.2.3.loccof=>cof}
	Let $\modelcat$ be a right proper cellular model category.  If $K$
	is a \emph{set} of objects in $\modelcat$, then every $K$-colocal cofibration
	$i:A\rightarrow B$ 
	is a cofibration in $\modelcat$.
\end{lem}
\begin{proof}
	Proposition \ref{prop1.2.weq-are-local} implies that every weak equivalence
	in $\modelcat$ is a $K$-colocal equivalence.  Therefore
	the class of trivial fibrations in $\modelcat$ is contained
	in the class of maps which are both fibrations in $\modelcat$
	and $K$-colocal equivalences.  So any map
	$i:A\rightarrow B$ having the left lifting property with respect to the class of maps
	that are both fibrations in $\modelcat$ and $K$-colocal equivalences,
	has also the left lifting property with respect to the class
	of trivial fibrations in $\modelcat$, and this implies
	that $i$ is a cofibration in $\modelcat$.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lem}
		\label{lem1.2.3.loccof&we<=>trivcof}
	Let $\modelcat$ be a right proper cellular model category.
	If $K$ is a \emph{set} of objects in $\modelcat$, then
	a map $i:A\rightarrow B$ is both a $K$-colocal cofibration
	and a $K$-colocal equivalence if and only if it is a
	trivial cofibration in $\modelcat$.
\end{lem}
\begin{proof}
	Assume that $i:A\rightarrow B$ is both a $K$-colocal cofibration
	and a $K$-colocal equivalence.  Factor $i$ as
	$\xymatrix{A \ar[r]^-{j}& C \ar[r]^-{p}& B}$, where $j$ is a trivial
	cofibration in $\modelcat$ and $p$ is a fibration in $\modelcat$.
	Proposition \ref{prop1.2.weq-are-local} implies that $j$ is a
	$K$-colocal equivalence, and since $K$-colocal equivalences have the
	two out of three property it follows that $p$ is both a fibration in 
	$\modelcat$ and a $K$-colocal equivalence.  Thus, $i$ has the left
	lifting property with respect to $p$, and the retract argument
	(see proposition \ref{prop1.1.retract}) implies that $i$
	is a retract of $j$, therefore $i$ is also a trivial cofibration in
	$\modelcat$.
	
	For the converse, assume that $i$ is a trivial cofibration in $\modelcat$,
	then proposition \ref{prop1.2.weq-are-local} implies that in particular
	$i$ is a $K$-colocal equivalence.  To finish the argument, just notice
	that $i$ being a cofibration implies that $i$ has the left lifting
	property with respect to the class of fibrations in $\modelcat$, so
	in particual $i$ has the left lifting property with respect to the class
	of maps in $\modelcat$ which are both fibrations in $\modelcat$ and
	$K$-colocal equivalences.  This shows that $i$ is a
	$K$-colocal cofibration.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{prop}
		\label{prop1.2.3.trivcof-fib-fac-rightBousloc}
	Let $\modelcat$ be a right proper cellular model category.
	If $K$ is a \emph{set} of objects of $\modelcat$, then there is
	a functorial factorization for every map $i:A\rightarrow B$ in
	$\modelcat$ as $\xymatrix{A \ar[r]^-{j}& C \ar[r]^-{p}& B}$,
	where $j$ is both a $K$-colocal cofibration and
	a $K$-colocal equivalence, and $p$ is a fibration in
	$\rightBousloc$.
\end{prop}
\begin{proof}
	By lemma \ref{lem1.2.3.loccof&we<=>trivcof}, the trivial cofibrations in $\modelcat$
	and the class of maps which are both $K$-colocal cofibrations and $K$-colocal equivalences
	coincide.  By construction (see definition \ref{def1.2.1.rightBousloc}) the fibrations
	in $\modelcat$ and the fibrations in $\rightBousloc$ coincide.
	Therefore since $\modelcat$ satisfies axiom $\mathbf{MC5}$, we get the functorial
	factorization $\xymatrix{A \ar[r]^-{j}& C \ar[r]^-{p}& B}$ that we were
	looking for.
\end{proof}

%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%
\begin{lem}
		\label{lem1.2.3.class-K-colocal-cofs}
	Let $\modelcat$ be a right proper cellular model category, and
	let $K$ be a \emph{set} of objects in $\modelcat$.
	If $i:A\rightarrow B$ is a cofibration in $\modelcat$,
	$j:B\rightarrow C$ is a weak equivalence in $\modelcat$,
	and $ji:A\rightarrow C$ is a $K$-colocal cofibration,
	then $i$ is a $K$-colocal cofibration.
\end{lem}

%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%
\begin{prop}
		\label{prop1.2.3.cof-trivfib-fact-rightBousloc}
	Let $\modelcat$ be a right proper cellular model category.
	If $K$ is a set of objects in $\modelcat$, then there is a functorial
	factorization for every map $j:A\rightarrow B$ in $\modelcat$
	as $\xymatrix{A \ar[r]^-{i}& C \ar[r]^-{q}& B}$ where
	$i$ is a $K$-colocal cofibration and $q$ is both a $K$-colocal
	equivalence and a fibration in $\modelcat$.
\end{prop}
\end{section}

